Analyzing Multi-Task Learning for Abstractive Text Summarization

Despite the recent success of multi-task learning and pre-finetuning for natural language understanding, few works have studied the effects of task families on abstractive text summarization. Task families are a form of task grouping during the pre-finetuning stage to learn common skills, such as reading comprehension. To close this gap, we analyze the influence of multi-task learning strategies using task families for the English abstractive text summarization task. We group tasks into one of three strategies, i.e., sequential, simultaneous, and continual multi-task learning, and evaluate trained models through two downstream tasks. We find that certain combinations of task families (e.g., advanced reading comprehension and natural language inference) positively impact downstream performance. Further, we find that choice and combinations of task families influence downstream performance more than the training scheme, supporting the use of task families for abstractive text summarization.

==> tables/RQ2/RQ2.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Results for Research Question 2}
    \label{tab:results_standard_comb}
\end{table}

==> tables/RQ3/Q4-combination_selection.tex <==
\begin{table}[htbp]
    \centering
    \small
    \begin{tabular}{l l l}
        \toprule
       \textbf{good SUM pairings} & \textbf{good family pairings} & \textbf{resulting pairings}  \\
       \midrule
        RC, CMNS & CMNS\&CBQA, RC\&CLS & SUM+RC+CMNS, SUM+CMNS+CBQA, SUM+RC+CLS \\
        C & D \\
        C & D \\
        C & D \\
        \bottomrule
    \end{tabular}
    \caption{Combinations for Q4.}
    \label{tab:q4_combinations}
\end{table}

==> tables/RQ3/RQ3.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{c|c}
         &  \\
         & 
    \end{tabular}
    \caption{Results for Research Question 3}
    \label{tab:results_proposed_comb}
\end{table}

==> tables/finetuning_selection.tex <==
\begin{table}[htbp]
\small
\resizebox{\columnwidth}{!}{
    \begin{tabular}{lll}
    \toprule
\textbf{Task  }          & \textbf{Characteristic   }                                                  & \textbf{Database}                                                                                                 \\ \midrule
CNN / DailyMail & news                                                               & CNN                                                                                                      \\
Reddit TIFU     & blog / comment                                                     & Reddit                                                                                                   \\
WikiHow         & tutorials                                                          & WikiHow                                                                                                  \\
BigPatent       & patents                                                            & \begin{tabular}[c]{@{}l@{}}U.S. patent documents with human\\ written abstractive summaries\end{tabular} \\
arXiv           & scientific paper                                                   & arXiv                                                                                                    \\
PubMed          & \begin{tabular}[c]{@{}l@{}}scientific paper\\ medical\end{tabular} & PubMed                                                                                                   \\ \hdashline
XSum            & news                                                               & BBC articles (2010 to 2017) \\
\bottomrule

\end{tabular}
}
    \caption{List of finetuning tasks + characteristics + database}
    \label{tab:finetuning_selection}
\end{table}
\begin{table}[]

\end{table}
